BanglaNum -- A Public Dataset for Bengali Digit Recognition from Speech

Automatic speech recognition (ASR) converts the human voice into readily understandable and categorized text or words. Although Bengali is one of the most widely spoken languages in the world, there have been very few studies on Bengali ASR, particularly on Bangladeshi-accented Bengali. In this study, audio recordings of spoken digits (0-9) from university students were used to create a Bengali speech digits dataset that may be employed to train artificial neural networks for voice-based digital input systems. This paper also compares the Bengali digit recognition accuracy of several Convolutional Neural Networks (CNNs) using spectrograms and shows that a test accuracy of 98.23% is achievable using parameter-efficient models such as SqueezeNet on our dataset.

==> tables/hyperparamers.tex <==
\begin{table}[ht]
\centering
\caption{Hyperparameter Search}
\footnotesize
%\small
%\normalsize
\label{table:hyperparameter}
\begin{tabular}{|lll|ll|ll|}
\hline
\multicolumn{3}{|l|}{\textbf{Hyperparameters}}                                              & \multicolumn{2}{l|}{\textbf{Basic CNN}}                   & \multicolumn{2}{l|}{\textbf{SqueezeNet}}                  \\ \hline
\multicolumn{1}{|l|}{\textbf{Batch}} & \multicolumn{1}{l|}{\textbf{Window}} & \textbf{Step} & \multicolumn{1}{l|}{\textbf{Val Acc}} & \textbf{Test Acc} & \multicolumn{1}{l|}{\textbf{Val Acc}} & \textbf{Test Acc} \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{512}             & 256           & \multicolumn{1}{l|}{0.9742}           & 0.9688            & \multicolumn{1}{l|}{0.8454}           & 0.8086            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{512}             & 128           & \multicolumn{1}{l|}{0.9691}           & 0.9688            & \multicolumn{1}{l|}{0.9175}           & 0.9375            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{512}             & 64            & \multicolumn{1}{l|}{0.9639}           & 0.9492            & \multicolumn{1}{l|}{0.9588}           & 0.9609            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{512}             & 32            & \multicolumn{1}{l|}{0.9639}           & 0.9531            & \multicolumn{1}{l|}{0.9588}           & 0.9609            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{256}             & 128           & \multicolumn{1}{l|}{0.9794}           & 0.9648            & \multicolumn{1}{l|}{0.9536}           & 0.9297            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{256}             & 64            & \multicolumn{1}{l|}{0.9794}           & 0.9648            & \multicolumn{1}{l|}{0.9536}           & 0.9531            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{256}             & 32            & \multicolumn{1}{l|}{0.9691}           & 0.9727            & \multicolumn{1}{l|}{0.9691}           & 0.9688            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{128}             & 64            & \multicolumn{1}{l|}{0.9691}           & 0.9531            & \multicolumn{1}{l|}{0.9433}           & 0.9531            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{128}             & 32            & \multicolumn{1}{l|}{0.9794}           & 0.9648            & \multicolumn{1}{l|}{0.9639}           & 0.9648            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{128}             & 16            & \multicolumn{1}{l|}{0.9691}           & 0.9688            & \multicolumn{1}{l|}{0.9536}           & 0.9688            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{64}              & 32            & \multicolumn{1}{l|}{0.9742}           & 0.9492            & \multicolumn{1}{l|}{0.9433}           & 0.9414            \\ \hline
\multicolumn{1}{|l|}{256}            & \multicolumn{1}{l|}{64}              & 16            & \multicolumn{1}{l|}{0.9588}           & 0.9492            & \multicolumn{1}{l|}{0.9485}           & 0.9219            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{512}             & 256           & \multicolumn{1}{l|}{0.9845}           & 0.9648            & \multicolumn{1}{l|}{0.8969}           & 0.875             \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{512}             & 128           & \multicolumn{1}{l|}{0.9742}           & 0.9570            & \multicolumn{1}{l|}{0.9691}           & 0.9688            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{512}             & 64            & \multicolumn{1}{l|}{0.9588}           & 0.9609            & \multicolumn{1}{l|}{0.9794}           & 0.9609            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{512}             & 32            & \multicolumn{1}{l|}{0.9691}           & 0.9531            & \multicolumn{1}{l|}{0.9845}           & 0.9688            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{256}             & 128           & \multicolumn{1}{l|}{0.9845}           & 0.9688            & \multicolumn{1}{l|}{0.9639}           & 0.9688            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{256}             & 64            & \multicolumn{1}{l|}{0.9845}           & 0.9766            & \multicolumn{1}{l|}{0.9639}           & 0.9609            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{256}             & 32            & \multicolumn{1}{l|}{0.9742}           & 0.9766            & \multicolumn{1}{l|}{0.9845}           & 0.9766            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{128}             & 64            & \multicolumn{1}{l|}{0.9794}           & 0.9414            & \multicolumn{1}{l|}{0.9433}           & 0.9531            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{128}             & 32            & \multicolumn{1}{l|}{0.9691}           & 0.9766            & \multicolumn{1}{l|}{0.9639}           & 0.9805            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{128}             & 16            & \multicolumn{1}{l|}{0.9691}           & 0.9531            & \multicolumn{1}{l|}{0.9794}           & 0.9727            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{64}              & 32            & \multicolumn{1}{l|}{0.9639}           & 0.9648            & \multicolumn{1}{l|}{0.9381}           & 0.9375            \\ \hline
\multicolumn{1}{|l|}{128}            & \multicolumn{1}{l|}{64}              & 16            & \multicolumn{1}{l|}{0.9691}           & 0.9375            & \multicolumn{1}{l|}{0.9175}           & 0.9062            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{512}             & 256           & \multicolumn{1}{l|}{0.9845}           & 0.9531            & \multicolumn{1}{l|}{0.9691}           & 0.9336            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{512}             & 128           & \multicolumn{1}{l|}{0.9845}           & 0.9492            & \multicolumn{1}{l|}{0.9485}           & 0.9375            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{512}             & 64            & \multicolumn{1}{l|}{0.9845}           & 0.9531            & \multicolumn{1}{l|}{0.9948}           & 0.9805            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{512}             & 32            & \multicolumn{1}{l|}{0.9691}           & 0.9414            & \multicolumn{1}{l|}{0.9897}           & 0.9609            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{256}             & 128           & \multicolumn{1}{l|}{0.9897}           & 0.9570            & \multicolumn{1}{l|}{0.9794}           & 0.957             \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{256}             & 64            & \multicolumn{1}{l|}{0.9897}           & 0.9648            & \multicolumn{1}{l|}{0.9897}           & 0.9648            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{256}             & 32            & \multicolumn{1}{l|}{0.9897}           & 0.9531            & \multicolumn{1}{l|}{0.9948}           & 0.9609            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{128}             & 64            & \multicolumn{1}{l|}{0.9845}           & 0.9688            & \multicolumn{1}{l|}{0.9897}           & 0.9453            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{128}             & 32            & \multicolumn{1}{l|}{0.9897}           & 0.9531            & \multicolumn{1}{l|}{0.9897}           & 0.9531            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{128}             & 16            & \multicolumn{1}{l|}{0.9845}           & 0.9375            & \multicolumn{1}{l|}{0.9897}           & 0.9727            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{64}              & 32            & \multicolumn{1}{l|}{0.9691}           & 0.9609            & \multicolumn{1}{l|}{0.9536}           & 0.9609            \\ \hline
\multicolumn{1}{|l|}{64}             & \multicolumn{1}{l|}{64}              & 16            & \multicolumn{1}{l|}{0.9536}           & 0.9336            & \multicolumn{1}{l|}{0.9794}           & 0.9570            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{512}             & 256           & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9554}           & 0.9292            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{512}             & 128           & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9821}           & 0.9690            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{512}             & 64            & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9955}           & 0.9690            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{512}             & 32            & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9955}           & 0.9779            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{256}             & 128           & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9821}           & 0.969             \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{256}             & 64            & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9911}           & 0.9602            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{256}             & 32            & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9955}           & 0.9823            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{128}             & 64            & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9911}           & 0.9690            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{128}             & 32            & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{1.0000}           & 0.9735            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{128}             & 16            & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9955}           & 0.9735            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{64}              & 32            & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9821}           & 0.9823            \\ \hline
\multicolumn{1}{|l|}{32}             & \multicolumn{1}{l|}{64}              & 16            & \multicolumn{1}{l|}{}                 &                   & \multicolumn{1}{l|}{0.9911}           & 0.9602            \\ \hline
\end{tabular}
\end{table}
